Approximability of TSP on Power Law Graphs

In this paper we study the special case of Graphic TSP where the underlying graph is a power law graph (PLG). We give a refined analysis of some of the current best approximation algorithms and show that an improved approximation ratio can be achieved for certain ranges of the power law exponent $\beta$. For the value of power law exponent $\beta=1.5$ we obtain an approximation ratio of $1.34$ for Graphic TSP. Moreover we study the $(1,2)$-TSP with the underlying graph of $1$-edges being a PLG. We show improved approximation ratios in the case of underlying deterministic PLGs for $\beta$ greater than $1.666$. For underlying random PLGs we further improve the analysis and show even better expected approximation ratio for the range of $\beta$ between $1$ and $3.5$. On the other hand we prove the first explicit inapproximability bounds for $(1,2)$-TSP for an underlying power law graph.

==> PlotLowerBound2.tex <==
\begin{asy}
 defaultpen(fontsize(11));
 import graph;
 import gsl;
     size(13cm,9cm,IgnoreAspect);
     

     pen dashed=linetype(new real[] {4,4});
     pen p=linewidth(.75);

     //real f(real x) {return (3^(x)*516*(zeta(x)+1)+1)/(3^(x)*516*(zeta(x)+1));}
     real f(real x) {return (3^(x)*516*(zeta(x)+1/2)+1)/(3^(x)*516*(zeta(x)+1/2));}
     pair F(real x) {return (x,f(x));}
     //real g(real x) {return ((zeta(x)+1)*3^(x-1)*2(x-1)*354+1)/((zeta(x)+1)*3^(x-1)*2(x-1)*354);}
     real g(real x) {return (4^(x)*36*(zeta(x)+1/2)+1)/(4^(x)*36*(zeta(x)+1/2));}
     pair G(real x) {return (x,g(x));}
     //real h(real x) {return 535/534;}
  
     draw("$$",graph(f,1.1,9.5),p);
     draw("$$",graph(g,1.1,9.5),dashed+p);
     //draw("$$",graph(h,1.1,3),dotted+p);
     //draw("$$",graph(i,1.1,3),dotted+p);
     //draw("$\frac{535}{534}$",graph(h,1.1,3),dotted+p);
     
 //    ylimits(1.968,2);
     xaxis("$\beta$",BottomTop,LeftTicks);
     yaxis("lower bound",LeftRight,RightTicks);
     //label("$\frac{3^{\beta}\cdot 516\cdot (\zeta (\beta)+\frac{1}{2})+1}{3^{\beta}\cdot 516\cdot (\zeta (\beta)+\frac{1}{2})}$",F(1.5),N);
     //label("$\frac{(\zeta (\beta)+\frac{1}{2})\cdot 3^{\beta -1}\cdot 2(\beta -1)\cdot 354+1}{(\zeta (\beta)+\frac{1}{2})\cdot 3^{\beta -1}\cdot 2(\beta -1)\cdot 354}$",G(1.75),NE);

     //attach(legend(),(point(S).x,truepoint(S).y),10S,UnFill);
  \end{asy}

